Monitoring and Verification of Multitenant Kubernetes Clusters using TLA+ Trace Checking

In distributed systems, model checking is usually used at design time for specifying an abstract model of the system and then exhaustively checking all possible behaviors. TLA+ is commonly used in this way as a specification language, together with the TLC model checker. In this paper, we present a monitoring tool that, at its core, utilizes TLA+ specifications in a different way. The tool utilizes a TLA+ trace-checking specification to detect violations in behavior inferred from Kubernetes audit logs. Our primary use case focuses on multitenancy violations; however, the pipeline is not limited to that setting. Specifically, it demonstrates how formal reasoning can be incorporated into live Kubernetes environments to improve monitoring and correctness checking.

==> eptcsdata.tex <==
\providecommand{\firstpage}{51}
\providecommand{\publicationstatus}{Mircea Marin, Adrian Cr\u{a}ciun (Eds.): FROM 2026\\
EPTCS 452, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.452.4}{10.4204/EPTCS.452.4}}

